Post-hoc Probabilistic Vision-Language Models

Vision-language models (VLMs), such as CLIP and SigLIP, have found remarkable success in classification, retrieval, and generative tasks. For this, VLMs deterministically map images and text descriptions to a joint latent space in which their similarity is assessed using the cosine similarity. However, a deterministic mapping of inputs fails to capture uncertainties over concepts arising from domain shifts when used in downstream tasks. In this work, we propose post-hoc uncertainty estimation in VLMs that does not require additional training. Our method leverages a Bayesian posterior approximation over the last layers in VLMs and analytically quantifies uncertainties over cosine similarities. We demonstrate its effectiveness for uncertainty quantification and support set selection in active learning. Compared to baselines, we obtain improved and well-calibrated predictive uncertainties, interpretable uncertainty estimates, and sample-efficient active learning. Our results show promise for safety-critical applications of large-scale models.

==> figs/process_diagram.tex <==
\begin{tikzpicture}
			
  \newcommand{\encoder}[4]{%
    \begin{scope}[xshift=#3cm, yshift=#4cm]
      \fill[#1] (0,0) -- (0,3*#2) -- (1,2*#2) -- (1,-2*#2) -- (0,-3*#2) -- cycle;
    \end{scope}
  }
  
  \newcommand{\dist}[6]{%
    \begin{scope}[xshift=#2cm, yshift=#3cm, fill opacity=0.25]
      \draw[rotate=#4, thick, #1!60, fill=#1!60, #6] (0, 0) ellipse (#5);
      \draw[rotate=#4, thick, #1!90, fill=#1!90, scale=0.5, #6] (0, 0) ellipse (#5);
      \draw[rotate=#4, thick, draw=#1, fill=#1, scale=0.5*0.25, #6] (0, 0) ellipse (#5);
    \end{scope}
  }
  
  \pgfmathdeclarefunction{gauss}{2}{%
    \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
  }
  
  % draw input images
  \node[draw=scYellow, thick, anchor=east] at (-2.8,0) {\includegraphics[width=1cm]{pics/homeoffice-product_test_mutual_info_highest_3.png}};
  \node[draw=scBlue, thick, anchor=east] at (-1.4,0) {\includegraphics[width=1cm]{pics/homeoffice-product_test_mutual_info_lowest_3.png}};
  \node[draw=scRed, thick, anchor=east] at (0,0) {\includegraphics[width=1cm]{pics/homeoffice-product_test_mutual_info_highest_4.png}};
  
  % draw input sentences
  \node[draw=scPurple, thick, dashed, align=center, anchor=east] at (0,-1.5) {\small An image of \{reading glasses\}.};
  \node[draw=scGreen, thick, dashed, align=center, anchor=east] at (0,-2.25) {\small An image of \{scissors\}.};
  \node[draw=scCyan, thick, dashed, align=center, anchor=east] at (0,-3) {\small An image of \{crayon pencils\}.};
  
  % draw encoders
  \encoder{black!20, draw=black!60}{0.25}{1}{0}
  \node at (1.5,0) {\small $\phi$};
  \encoder{black!20, draw=black!60}{0.25}{1}{-2.25}
  \node at (1.5,-2.25) {\small $\psi$};
  
  % draw lines connecting inputs and encoders
  \draw[-latex, scYellow] (-3.4, 0.6) to [out=15,in=140] (0.95,0.25);
  \draw[-latex, scBlue] (-2,-0.6) to [out=-15, in=220] (0.95,-.25);
  \draw[-latex, scRed] (0,0) to [out=0, in=180] (0.95,0);
  
  \draw[-latex, scPurple] (0,-1.5) to [out=0,in=140] (0.95,-2);
  \draw[-latex, scGreen] (0,-2.25) to [out=0,in=180] (0.95,-2.25);
  \draw[-latex, scCyan] (0,-3) to [out=0,in=220] (0.95,-2.5);
  
  % draw distribution over projection matrices
  % 1.5cm height * 0.25 scale = 0.375cm
  \begin{scope}[yshift=-0.125cm, xshift=4.5cm]
    \node at (-0.8,0.125) {\small $\phi(\bx^{\img}_i) \, \times$};
    \node at (0.5, 1) {\scriptsize $\distNorm(\bP,
    \bSigma_{\img})$ };
    
    % first column
    \pic[scale=0.25, fill=scRed] at (0, 0.375) {gauss=0.5/0.5};
    \pic[scale=0.25, fill=scRed] at (0, 0) {gauss=-0.5/0.5};
    \pic[scale=0.25, fill=scRed] at (0, -0.375) {gauss=0.5/0.3};
    % second column
    \pic[scale=0.25, fill=scRed] at (0.5, 0.375) {gauss=1/0.2};
    \pic[scale=0.25, fill=scRed] at (0.5, 0) {gauss=0.25/0.4};
    \pic[scale=0.25, fill=scRed] at (0.5, -0.375) {gauss=0/0.3};
    % third column
    \pic[scale=0.25, fill=scRed] at (0.5*2, 0.375) {gauss=0/0.3};
    \pic[scale=0.25, fill=scRed] at (0.5*2, 0) {gauss=1.5/0.7};
    \pic[scale=0.25, fill=scRed] at (0.5*2, -0.375) {gauss=-0.5/0.5};
  \end{scope}
  
  \begin{scope}[yshift=-2.375cm, xshift=4.5cm]
    \node at (-0.8,0.125) {\small $\psi(\bx^{\txt}_i) \, \times$};
    \node at (0.5, 1) {\scriptsize $\distNorm(\bQ,
    \bSigma_{\txt})$ };
    
    % first column
    \pic[scale=0.25, fill=scRed] at (0, 0.375) {gauss=1/0.5};
    \pic[scale=0.25, fill=scRed] at (0, 0) {gauss=-0.5/0.2};
    \pic[scale=0.25, fill=scRed] at (0, -0.375) {gauss=-0.5/0.5};
    % second column
    \pic[scale=0.25, fill=scRed] at (0.5, 0.375) {gauss=1/0.4};
    \pic[scale=0.25, fill=scRed] at (0.5, 0) {gauss=0.5/0.2};
    \pic[scale=0.25, fill=scRed] at (0.5, -0.375) {gauss=-0.1/0.3};
    % third column
    \pic[scale=0.25, fill=scRed] at (0.5*2, 0.375) {gauss=1/0.5};
    \pic[scale=0.25, fill=scRed] at (0.5*2, 0) {gauss=.5/0.7};
    \pic[scale=0.25, fill=scRed] at (0.5*2, -0.375) {gauss=0/0.5};
  \end{scope}
  
  \draw[-latex, thick] (2,0) -- (2.9, 0);
  \draw[-latex, thick] (2,-2.25) -- (2.9, -2.25);
  
  \begin{scope}[xshift=4cm]
    
    % draw distributions over feature projections
    \begin{scope}[xshift=0.5cm]
      \dist{scRed}{3.2}{-0.3}{0}{0.75cm and 0.5cm}{} % scissors (hard)
      \dist{scYellow}{3}{0}{45}{0.75cm and 0.25cm}{} % scissors
      \dist{scBlue}{3.8}{0.4}{-30}{0.4cm and 0.2cm}{} % reading glasses
      
      \begin{scope}[yshift=-2.25cm]
        \dist{scCyan}{3.2}{-.4}{-45}{0.4cm and 0.5cm}{dashed} % crayon pencils
        \dist{scPurple}{3.7}{0.3}{22}{0.5cm and 0.3cm}{dashed} % reading glasses
        \dist{scGreen}{2.8}{0.1}{15}{0.25cm and 0.15cm}{dashed} % scissors
      \end{scope}
    \end{scope}
    
    % draw lines connecting encoders and distributions
    \draw[-latex, thick] (2,0) -- (2.9, 0);
    \draw[-latex, thick] (2,-2.25) -- (2.9, -2.25);
    
    \draw[-latex, thick] (5, 0) -- (5.9, 0);
    \draw[-latex, thick] (5, 0) -- (5.9, -1.025);
    \draw[-latex, thick] (5, 0) -- (5.9, -2.15);
    
    \draw[-latex, thick, dashed] (5, -2.25) -- (5.9, -0.1);
    \draw[-latex, thick, dashed] (5, -2.25) -- (5.9, -1.225);
    \draw[-latex, thick, dashed] (5, -2.25) -- (5.9, -2.25);
    
    % draw distributions over cosine similarities
    \begin{scope}[xshift=6cm]
      
      \begin{scope}[yshift=-0.5cm]
        \begin{axis}[
          no markers, domain=0:10, samples=100,
          height=2.5cm, width=4cm,
          xtick=\empty, ytick=\empty,
          axis line style={draw=scPurple, dashed, thick},
          axis background/.style={fill=scPurple!10}
          ]
          \addplot [very thick, scRed] {gauss(2,1.25)};
          \addplot [very thick, scYellow] {gauss(4,0.75)};
          \addplot [very thick, scBlue] {gauss(8,0.4)};
        \end{axis}
      \end{scope}
      
      \begin{scope}[yshift=-1.625cm]
        \begin{axis}[
          no markers, domain=0:10, samples=100,
          height=2.5cm, width=4cm,
          xtick=\empty, ytick=\empty,
          axis line style={draw=scGreen, dashed, thick},
          axis background/.style={fill=scGreen!10}
          ]
          \addplot [very thick, scBlue] {gauss(2,0.25)};
          \addplot [very thick, scRed] {gauss(5.5,1)};
          \addplot [very thick, scYellow] {gauss(7,0.5)};
        \end{axis}
      \end{scope}
      
      \begin{scope}[yshift=-2.75cm]
        \begin{axis}[
          no markers, domain=0:10, samples=100,
          height=2.5cm, width=4cm,
          xtick=\empty, ytick=\empty,
          axis line style={draw=scCyan, dashed, thick},
          axis background/.style={fill=scCyan!10}
          ]
          \addplot [very thick, scRed] {gauss(6,1.75)};
          \addplot [very thick, scYellow] {gauss(2,1)};
          \addplot [very thick, scBlue] {gauss(1.5,0.5)};
        \end{axis}
      \end{scope}
    \end{scope}
    
    % draw labels
    
    \node[align=center, anchor=north] at (3.7, 2) {\small Embeddings Become\\ \small Probabilistic  (\cref{eq:feature_dist})};
    \node[align=center, anchor=north] at (7.2, 2) {\small Cosine Similarities Become\\ \small Probabilistic (\cref{eq:cosine_sim_dist}) };
  \end{scope}
  
  \node[, anchor=north] at (-2, 2) {\small Inputs};
  \node[anchor=north, align=center] at (1.5, 2) {\small Encoders \\ \small \faLock};
  
  \node[align=center, anchor=north] at (4.5, 2) {\small Laplace Approx.\\ \small (\cref{eq:hessian})};
  
\end{tikzpicture}


==> figs/teaser3-update.tex <==
%!TEX root = ../main.tex
\newcommand{\arcarrow}[8]% inner radius, middle radius, outer radius, start angle, end angle, tip protusion angle, options, text
{   \pgfmathsetmacro{\rin}{#1}
    \pgfmathsetmacro{\rmid}{#2}
    \pgfmathsetmacro{\rout}{#3}
    \pgfmathsetmacro{\astart}{#4}
    \pgfmathsetmacro{\aend}{#5}
    \pgfmathsetmacro{\atip}{#6}
    \fill[#7,draw=white,line width=1pt] (\astart:\rin) arc (\astart:\aend:\rin) -- (\aend+\atip:\rmid) -- (\aend:\rout) arc (\aend:\astart:\rout) -- (\astart+\atip:\rmid) -- cycle;
    \path[decoration={text along path, text={#8}, text align={align=center}, raise=-0.5ex},decorate] (\astart+\atip:{\rmid-.05}) arc (\astart+\atip:\aend+\atip:{\rmid-.05});
}
\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}
% \tikzexternalenable
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
        box/.style={minimum width=0.485\textwidth,minimum height=2.9cm,rounded corners=4pt,text width=3cm,align=center,fill=white}, 
        label/.style = {font={\footnotesize},anchor=north,inner sep=0pt,align=center}, 
    ]

  \node[box, minimum width=0.45\columnwidth, draw=black!30,fill=blue!03] (part1) at (0,0) {};
  %\node[box,minimum width=0.38\columnwidth,draw=black!30,fill=blue!03] (part2) at (6.5cm,0) {};
  \node[box,minimum width=0.38\columnwidth,draw=black!30,fill=blue!03] (part3) at (12cm,0) {};
  \node[box,minimum width=0.38\columnwidth,draw=black!30,fill=blue!03] (part2) at ($(part1.east)!.5!(part3.west)$) {};

  \node[label] (label1) at ([yshift=-0.1cm]part1.north) {{\bf Post-hoc Probabilistic Model} };
  \node[label] (label2) at ([yshift=-0.1cm]part2.north) {{\bf Uncertainty Quantification} };
  \node[label] (label3) at ([yshift=-0.1cm]part3.north) {{\bf Active Learning}};
  
  % Add arrows
  \node[
    draw=black!30,
    fill=black!30,
    single arrow,
    shape border rotate=0,
    minimum height=1cm,
    single arrow head extend=0.25cm,
    rounded corners=1pt
  ] at ($(part1.east)!.5!(part2.west)$) {};
  \node[
    draw=black!30,
    fill=black!30,
    single arrow,
    shape border rotate=0,
    minimum height=1cm,
    single arrow head extend=0.25cm,
    rounded corners=1pt
  ] at ($(part2.east)!.5!(part3.west)$) {};
        
  
  
  % VLM 
  \pic[fill=gray, draw=gray, scale=1.5, transform shape] (vlm) at (-2, 0) {robothead};
  \node[align=center,font=\scriptsize] at (-2,-0.8) { Pre-trained VLM \\(CLIP, SigLIP)};

  %\draw[-latex,thick] (-1.1,0) -- node[sloped,above]{\scriptsize Hessian estimation} (1.2,0);
  \draw[->,thick] (-1.2,0) -- node[sloped,above,align=left]{\scriptsize Laplace approximation} (1.3,0);
  % \draw[-latex] (0.7,0) -- node[sloped,below]{\scriptsize \cref{sec:uncertainty_quantification}} (3.3,0);

  % Bayes VLM
  \pic[fill=scCyan, draw=scCyan, scale=1.5, transform shape] (bayes-vlm) at (2, 0) {expert};
  \node[align=center] (bayes) at (2,-0.7) {\scriptsize BayesVLM};
  %\node[align=center] (bayes) at (bayes-vlm.south) {\scriptsize BayesVLM};

  % UQ part
  \begin{scope}[xshift=6.5cm,yshift=0.5cm]
  \node[draw=scRed, thick, anchor=center,rounded corners=2pt,fill=white] (im0) at (-1.0,-.25) 
    {\includegraphics[width=1cm]{pics/homeoffice-product_test_mutual_info_highest_3.png}};
  \node[draw=scGreen, thick, anchor=center,rounded corners=2pt,fill=white] (im1) at (1.0,-.25) 
    {\includegraphics[width=1cm]{pics/homeoffice-product_test_mutual_info_lowest_3.png}};
% \node[align=center,font=\scriptsize] at (0.5, 1.0) {P(scissor)};
% \node[align=center,font=\scriptsize] at (1.5, 1.0) {P(glasses)};
%\node[align=center,font=\scriptsize] at (-2.0, -1.0) {Probability};
  \node[align=right,font=\scriptsize,below of=im0] {Glasses: 0.45 \\ Scissors: 0.55};
  \node[align=right,font=\scriptsize,below of=im1] {Glasses: 0.99 \\ Scissors: 0.01};
  \node[align=center,font=\scriptsize] at (-1, -1.75) {\bfseries \textcolor{scRed}{Uncertain}};
  \node[align=center,font=\scriptsize] at (1, -1.75) {\bfseries \textcolor{scGreen}{Certain}};
  
  \end{scope}
  
  
  % AL part
  \begin{scope}[xshift=12cm,yshift=0.5cm]
  
  \node[align=center,draw=scRed, thick, anchor=east, rounded corners=1pt, fill=white] 
    at (-1.25,0.2)
    {\includegraphics[width=0.5cm]{pics/scissor.png}};
  \node[align=center,draw=scRed, thick, anchor=east, rounded corners=1pt, fill=white] 
    at (-1.25,-0.6)
    {\includegraphics[width=0.5cm]{pics/homeoffice-product_test_mutual_info_highest_4.png}};
  \node[align=center,draw=scRed, thick, anchor=east, rounded corners=1pt, fill=white] 
    at (-1.25,-1.4)
    {\includegraphics[width=0.5cm]{pics/scissor2.png}};;
  
  %\node[align=center,font=\scriptsize] at (-1, -2.0) 
  %  {use {\bfseries uncertainty} to \\ select fine tuning data};
  \draw[->, thick] (-1,-0.6) -- (0.5,-0.6) node[midway, above] {\scriptsize Update model} node[midway, below,align=center,font=\tiny] {Use {\bfseries uncertainty} to \\ select fine tuning data};

  \node[align=center,draw=scGreen, thick, anchor=center, fill=white, rounded corners=2pt] (im2) at (1.5,-.25) {\includegraphics[width=1cm]{pics/homeoffice-product_test_mutual_info_highest_3.png}};
  \node[align=right,font=\scriptsize,below of=im2]  {Glasses: 0.2 \\ Scissors: 0.8};
  \node[align=center,font=\scriptsize] at (1.5, -1.75) {\bfseries \textcolor{scGreen}{More certain now}};
  \end{scope}

 % \begin{scope}[xshift=-3.75cm,yshift=-4cm]
 %   \begin{axis}[
 %     no markers, domain=0:10, samples=100,
 %     height=3cm, width=4cm,
 %     xtick=\empty, ytick=\empty,
 %     axis line style={draw=none},
 %     ymax=1,
 %     xlabel={\vspace{-2.5em}\scriptsize Distribution of Cosine Similarities},
 %     xlabel shift=-3.5pt,
 %     scale=1.4, % added for increasing size
 %     ]
 %     \addplot [very thick, scBlue] {gauss(2,1.25)};
 %     \addplot [very thick, scYellow] {gauss(4,0.75)};
 %     \addplot [very thick, scPurple] {gauss(8,0.4)};
 %     \coordinate (title_node) at (rel axis cs:0.5,1.6);
 %   \end{axis}
 % \end{scope}
%  
%  %\node[align=center, font=\scriptsize] (uq) at (title_node) {Uncertainty\\ Quantification};
%  % \node[align=center, font=\scriptsize, xshift=4.05cm] (al) at (title_node) {Active\\Learning};
%
%  %\draw[-latex] (bayes) -- node[left, font=\scriptsize]{\cref{sec:dist_cosine}} (uq);
%  % \draw[-latex] (bayes) -- node[left, font=\scriptsize]{} ([xshift=1.1cm,yshift=-0.75cm]title_node);
%  \draw[-latex,thick] (bayes) -- (part2.north east);
%  % \draw[-latex,thick] (bayes) -- ([xshift=-0.07cm]part3.north);
%  \draw[-latex,thick] ([xshift=-0.07cm, yshift=0.65cm]part3.north) -- ([xshift=-0.07cm]part3.north); % for making the line straight to 
%
%  
%  % \draw[-latex] (bayes) -- node[right, font=\scriptsize]{} ([xshift=-0.07cm,yshift=0.1cm]label3.north);
%
%  \begin{scope}[xshift=2.15cm, yshift=-3.3cm, 
%    scale=1.0, % added for increasing size
%    ]
%    \foreach \x/\y in {0/Estimation,120/Selection,240/Training} 
%    {  
%      % inner radius, middle radius, outer radius, start angle, end angle, tip protusion angle, options, text 
%      \arcarrow{0.5}{0.65}{0.8}{\x}{\x+120}{5}{scBlue!50}{|\tiny|\y}
%    }
%    % \end{scope}
%  \end{scope}

\end{tikzpicture}}


==> preamble.tex <==
% better colours
\usepackage{safecolours}

% custom colors
\colorlet{scBlue}{tol-colour1}
\colorlet{scRed}{tol-colour2}
\colorlet{scGreen}{tol-colour3}
\colorlet{scYellow}{tol-colour4}
\colorlet{scCyan}{tol-colour5}
\colorlet{scPurple}{tol-colour6}

% additional libraries
\usepackage{tikz}

% fontawesome for icons
\usepackage{fontawesome5}

% list of useful math definitions, helper function, and more...
\usepackage{shortex-light} % contains cleverref and hence needs to be loaded after hyperref

% additional function definitions
\newcommand{\todo}[1]{\emph{\color{scRed}#1}}

\newcommand{\trainset}{\mcD_{\text{train}}}
\newcommand{\testset}{\mcD_{\text{test}}}

\newcommand{\ntrain}{\ensuremath{n_{\text{train}}}}
\newcommand{\nval}{\ensuremath{n_{\text{val}}}}
\newcommand{\ntest}{\ensuremath{n_{\text{test}}}}
\newcommand{\nclass}{\ensuremath{c}}

% additional commands
\newcommand{\MAP}{\ensuremath{\operatorname{MAP}}}
\newcommand{\BALD}{\ensuremath{\operatorname{BALD}}}
\newcommand{\EPIG}{\ensuremath{\operatorname{EPIG}}}
\newcommand{\GGN}{\ensuremath{\operatorname{GGN}}}
\newcommand{\CE}{\ensuremath{\textsc{CE}}}
\newcommand{\img}{\ensuremath{\textsc{Img}}}
\newcommand{\txt}{\ensuremath{\textsc{Txt}}}
\newcommand{\enc}{\ensuremath{\textsc{Enc}}}
\newcommand{\imgtotxt}{\ensuremath{\img \rightarrow \txt}}
\newcommand{\txttoimg}{\ensuremath{\img \leftarrow \txt}}

\newcommand{\xstar}{\ensuremath{x^\star}}
\newcommand{\bxstar}{\ensuremath{\bx^\star}}
\newcommand{\ystar}{\ensuremath{y^\star}}
\newcommand{\bystar}{\ensuremath{\by^\star}}

\newcommand{\Var}{\mathbb{V}\mathrm{ar}}

% cosine similarity
\newcommand{\cossim}[2]{\ensuremath{\operatorname{S}_{\textsc{cos}}(#1, #2)}}

\newcommand{\softmax}[1]{\ensuremath{\operatorname{softmax}\left(#1\right)}}

% tikz specific definitions
\tikzset{
	oracle/.pic={
		\begin{scope}
			% Clip region scaled down
			\clip (-0.4,-0.195) rectangle (0.4, 0.4);
			% Draw the crystal ball outline, scaled down
			\fill[thick] (0, 0) circle (0.3);
		\end{scope}
		
		% Draw the base of the crystal ball with rounded corners (scaled down)
		\fill[rounded corners=0.075cm] (-0.3, -0.36) rectangle (0.3, -0.255);
		\fill[rounded corners=0.075cm] (-0.225, -0.3) rectangle (0.225, -0.225);
		
		% Adjusting and scaling down the star shape
		\begin{scope}[yshift=-0.2375cm, xshift=-0.17cm, scale=1.5]
			\fill[white] (0.18, 0.18) -- (0.195, 0.225) -- (0.24, 0.24) -- (0.195, 0.255) -- (0.18, 0.3) -- (0.165, 0.255) -- (0.12, 0.24) -- (0.165, 0.225) -- cycle;
		\end{scope}
	},
	robothead/.pic={
		
		% Draw the main head shape (scaled down)
		\fill[thick, rounded corners=0.1cm] (-0.3,-0.3) rectangle ++(0.6,0.6) ;
		
		% Draw the eyes (scaled down)
		\fill[white, thick] (-0.16,0.1) circle (0.08);
		\fill[white, thick] (0.16,0.1) circle (0.08);
		\fill[thick] (-0.16,0.1) circle (0.04);
		\fill[thick] (0.16,0.1) circle (0.04);
		
		% Draw the mouth (scaled down)
		\fill[white, thick, rounded corners=0.04cm] (-0.16,-0.16) rectangle ++(0.32,0.1);
		\draw[thick] (-0.08,-0.16) -- (-0.08,-0.06);
		\draw[thick] (0,-0.16) -- (0,-0.06);
		\draw[thick] (0.08,-0.16) -- (0.08,-0.06);
		
		% Draw the antenna (scaled down)
		\draw[thick] (0,0.3) -- (0,0.5);
		\fill[thick] (0,0.5) circle (0.04);
		
		% Draw the ears (scaled down)
		\fill[thick, rounded corners=0.04cm] (-0.4,0.1) rectangle ++(0.08,0.2);
		\fill[thick, rounded corners=0.04cm] (0.32,0.1) rectangle ++(0.08,0.2);
	},
	expert/.pic={
		
		% Draw the main head shape (scaled down)
		\fill[thick, rounded corners=0.1cm] (-0.3,-0.3) rectangle ++(0.6,0.6) ;
		
		% Draw the eyes (scaled down)
		\fill[white, thick] (-0.16,0.1) circle (0.08);
		\fill[white, thick] (0.16,0.1) circle (0.08);
		\fill[thick] (-0.16,0.1) circle (0.04);
		\fill[thick] (0.16,0.1) circle (0.04);
		
		% Draw thick black-framed square glasses
		\draw[thick, rounded corners=0.03cm, black] (-0.26, 0.02) rectangle ++(0.18, 0.16); % Left lens
		\draw[thick, rounded corners=0.03cm, black] (0.08, 0.02) rectangle ++(0.18, 0.16); % Right lens
		\draw[thick, black] (-0.08,0.1) -- (0.08,0.1); % Bridge
		\draw[thick, black] (-0.34,0.2) -- (-0.26,0.1); % Left frame extension
		\draw[thick, black] (0.34,0.2) -- (0.26,0.1); % Right frame extension	
		
		% Draw the mouth (scaled down)
		\fill[white, thick, rounded corners=0.04cm] (-0.16,-0.16) rectangle ++(0.32,0.1);
		\draw[thick] (-0.08,-0.16) -- (-0.08,-0.06);
		\draw[thick] (0,-0.16) -- (0,-0.06);
		\draw[thick] (0.08,-0.16) -- (0.08,-0.06);
		
		% Draw the antenna (scaled down)
		\draw[thick] (0,0.3) -- (0,0.5);
		\fill[thick] (0,0.5) circle (0.04);
		
		% Draw the ears (scaled down)
		\fill[thick, rounded corners=0.04cm] (-0.4,0.1) rectangle ++(0.08,0.2);
		\fill[thick, rounded corners=0.04cm] (0.32,0.1) rectangle ++(0.08,0.2);
	},	
	cross/.pic = {
		\draw[rotate = 45] (-#1,0) -- (#1,0);
		\draw[rotate = 45] (0,-#1) -- (0, #1);
	},
	pics/gauss/.style args={#1/#2}{
		code = {
			\begin{scope}
				\clip (-0.5,0) rectangle (1.5,1.5);
				\fill[black!10] (-0.5,0) rectangle (1.5,1.5);
				\fill[thick, domain=-10:10, samples=50] plot[smooth] (\x, {1/(#2*sqrt(2*pi))*exp(-(\x-#1)^2/(2*#2^2))});
				\draw[] (-0.5,0) rectangle (1.5,1.5);
			\end{scope}
		}
	}
}

==> prolip_table.tex <==

\begin{tabular}{l|l|ccccccc}
\toprule
Metrics & Methods & \sc Flowers-102 & \sc Food-101 & \sc CIFAR-10 & \sc CIFAR-100 & \sc ImageNet-R & \sc UCF101 & \sc SUN397 \\
\hline
   & Mean \citep{prolip} & \val{\bf}{77.83}{0.0053} & \val{\bf}{90.38}{0.0019} & \val{\bf}{96.52}{0.0018} & \val{\bf}{82.41}{0.0038} & \val{}{84.76}{0.0042} & \val{\bf}{69.94}{0.0033} & \val{\bf}{65.93}{0.0077}\\
\rowcolor{scCyan!30} \multirow{-2}{*}{\cellcolor{white}ACC $\uparrow$} & ProbCosine (\cref{eq:cosine_sim_dist}) & \val{\bf}{77.74}{0.0053} & \val{\bf}{90.35}{0.0019} & \val{\bf}{96.52}{0.0018} & \val{\bf}{82.48}{0.0038} & \val{\bf}{84.91}{0.0041} & \val{\bf}{69.99}{0.0033} & \val{\bf}{65.82}{0.0077}\\
 \hline
& Mean \citep{prolip} & \val{}{1.36}{0.0411} & \val{\bf}{0.33}{0.0060} & \val{\bf}{0.11}{0.0052} & \val{}{0.64}{0.0148} & \val{\bf}{0.59}{0.0164} & \val{}{1.05}{0.0120} & \val{}{1.28}{0.0316}\\
\rowcolor{scCyan!30} \multirow{-2}{*}{\cellcolor{white}NLPD $\downarrow$} & ProbCosine (\cref{eq:cosine_sim_dist}) & \val{\bf}{1.28}{0.0376} & \val{}{0.34}{0.0055} & \val{\bf}{0.11}{0.0047} & \val{\bf}{0.63}{0.0133} & \val{}{0.60}{0.0151} & \val{\bf}{1.02}{0.0108} & \val{\bf}{1.24}{0.0286}\\
 \hline
 & Mean \citep{prolip} & $5.31$ & $\bf0.79$ & $\bf0.60$ & $3.38$ & $\bf1.08$ & $5.99$ & $7.99$\\
\rowcolor{scCyan!30} \multirow{-2}{*}{\cellcolor{white}ECE $\downarrow$} & ProbCosine (\cref{eq:cosine_sim_dist}) & $\bf3.60$ & $2.57$ & $0.76$ & $\bf1.40$ & $3.53$ & $\bf2.23$ & $\bf4.73$\\

\bottomrule
\end{tabular}
    

==> zero_shot_openai.tex <==

\begin{tabular}{l|l|ccccc}
\toprule
Metrics & Methods & \sc Flowers-102 & \sc Food-101  & \sc EuroSAT  & \sc CIFAR-100 & \sc DTD \\
\hline
& CLIP~\cite{radford2021learning} & \val{\bf}{67.30}{0.60} & \val{}{86.14}{0.22} & \val{}{45.90}{0.55} & \val{\bf}{66.19}{0.47} & \val{\bf}{42.87}{1.14}\\
\multirow{3}{*}{\ACC} & CLIP (temp. scaling) & \val{\bf}{67.30}{0.60} & \val{}{86.14}{0.22} & \val{}{45.90}{0.55} & \val{\bf}{66.19}{0.47} & \val{\bf}{42.87}{1.14}\\
   & PCME++~\cite{pcmepp} & \val{}{40.59}{0.63} & \val{}{65.47}{0.30} & \val{}{28.83}{0.50} & \val{}{42.52}{0.49} & \val{}{23.30}{0.97}\\
 & PCME++ (\cref{eq:cosine_sim_dist}) & \val{}{40.43}{0.63} & \val{}{65.54}{0.30} & \val{}{28.83}{0.50} & \val{}{42.60}{0.49} & \val{}{23.19}{0.97}\\
 \rowcolor{scCyan!30}
 \cellcolor{white} & BayesVLM & \val{\bf}{67.49}{0.60} & \val{\bf}{86.45}{0.22} & \val{\bf}{46.68}{0.55} & \val{\bf}{66.10}{0.47} & \val{\bf}{42.87}{1.14}\\\hline
& CLIP~\cite{radford2021learning} & \val{}{1.67}{0.04} & \val{\bf}{0.48}{0.01} & \val{}{1.74}{0.02} & \val{\bf}{1.38}{0.01} & \val{}{2.16}{0.04}\\
 \multirow{3}{*}{\NLPD} & CLIP (temp. scaling) & \val{}{1.65}{0.04} & \val{}{0.48}{0.01} & \val{\bf}{1.73}{0.02} & \val{}{1.39}{0.01} & \val{}{2.15}{0.04}\\
 & PCME++~\cite{pcmepp} & \val{}{3.22}{0.05} & \val{}{1.30}{0.01} & \val{}{3.53}{0.03} & \val{}{2.28}{0.02} & \val{}{4.05}{0.07}\\
 & PCME++ (\cref{eq:cosine_sim_dist}) & \val{}{3.04}{0.04} & \val{}{1.25}{0.01} & \val{}{3.19}{0.03} & \val{}{2.21}{0.02} & \val{}{3.74}{0.06}\\
 \rowcolor{scCyan!30}
 \cellcolor{white}  & BayesVLM & \val{\bf}{1.61}{0.03} & \val{}{0.48}{0.01} & \val{\bf}{1.73}{0.02} & \val{}{1.41}{0.01} & \val{\bf}{2.13}{0.04}\\\hline
 & CLIP~\cite{radford2021learning} & $2.82$ & $3.41$ & $7.38$ & $11.18$ & $8.72$\\
 \multirow{3}{*}{\ECE} & CLIP (temp. scaling) & $3.35$ & $3.92$ & $7.02$ & $12.17$ & $8.06$\\
 & PCME++~\cite{pcmepp} & $8.81$ & $6.78$ & $34.87$ & $10.78$ & $25.95$\\
 & PCME++ (\cref{eq:cosine_sim_dist}) & $\bf2.79$ & $\bf1.54$ & $30.58$ & $\bf4.89$ & $19.18$\\
 \rowcolor{scCyan!30}
 \cellcolor{white}  & BayesVLM & $5.08$ & $5.28$ & $\bf6.55$ & $12.98$ & $\bf6.41$\\

\bottomrule
\end{tabular}
    

==> zero_shot_siglip.tex <==
% \begin{tabular}{l|l|ccccc}
% \toprule
% Metrics & Methods & \sc Flowers-102 & \sc Food-101  & \sc EuroSAT  & \sc CIFAR-100 & \sc DTD \\
% \hline
%     \multirow{3}{*}{\ACC} & SigLIP~\cite{zhai2023sigmoid} & \val{\bf}{82.31}{0.49} & \val{\bf}{88.81}{0.20} & \val{\bf}{40.74}{0.55} & \val{\bf}{71.27}{0.45} & \val{\bf}{63.62}{1.11}\\
%  & SigLIP (temp. scaling) & \val{\bf}{82.31}{0.49} & \val{\bf}{88.81}{0.20} & \val{\bf}{40.74}{0.55} & \val{\bf}{71.27}{0.45} & \val{\bf}{63.62}{1.11}\\
%  \rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM & \val{\bf}{82.40}{0.49} & \val{\bf}{88.87}{0.20} & \val{\bf}{40.72}{0.55} & \val{\bf}{71.22}{0.45} & \val{\bf}{63.67}{1.11}\\\hline
% \multirow{3}{*}{\NLPD} & SigLIP~\cite{zhai2023sigmoid} & \val{}{0.88}{0.03} & \val{\bf}{0.38}{0.01} & \val{}{1.98}{0.02} & \val{\bf}{1.08}{0.02} & \val{}{1.48}{0.05}\\
%  & SigLIP (temp. scaling) & \val{}{1.91}{0.01} & \val{}{1.64}{0.00} & \val{\bf}{1.86}{0.01} & \val{}{2.38}{0.01} & \val{}{2.20}{0.02}\\
%  \rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM & \val{\bf}{0.86}{0.03} & \val{\bf}{0.38}{0.01} & \val{}{1.95}{0.02} & \val{\bf}{1.08}{0.02} & \val{\bf}{1.46}{0.05}\\\hline
% \multirow{3}{*}{\ECE} & SigLIP~\cite{zhai2023sigmoid} & $\bf4.31$ & $\bf1.66$ & $15.95$ & $1.97$ & $8.19$\\
%  & SigLIP (temp. scaling) & $62.79$ & $65.83$ & $16.90$ & $57.79$ & $46.50$\\
%   \rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM & $4.49$ & $2.65$ & $\bf15.08$ & $\bf1.72$ & $\bf6.61$\\

% \bottomrule
% \end{tabular}

%% 
%% Rebuttal update
%% Results by Rui from 29.01.2025
%%
\begin{tabular}{l|l|ccccc}
\toprule
Metrics & Methods & \sc Flowers-102 & \sc Food-101  & \sc EuroSAT  & \sc CIFAR-100 & \sc DTD \\
\hline
    \multirow{5}{*}{ACC} & CLIP~\cite{radford2021learning} & \val{\bf}{82.31}{0.49} & \val{\bf}{88.81}{0.20} & \val{\bf}{40.74}{0.55} & \val{\bf}{71.27}{0.45} & \val{\bf}{63.62}{1.11}\\
 & CLIP (temp. scaling) & \val{\bf}{82.31}{0.49} & \val{\bf}{88.81}{0.20} & \val{\bf}{40.74}{0.55} & \val{\bf}{71.27}{0.45} & \val{\bf}{63.62}{1.11}\\
\rowcolor{scCyan!30}
\cellcolor{white} & BayesVLM & \val{\bf}{82.40}{0.49} & \val{\bf}{88.87}{0.20} & \val{\bf}{40.72}{0.55} & \val{\bf}{71.22}{0.45} & \val{\bf}{63.67}{1.11}\\\hline
\multirow{5}{*}{NLPD} & CLIP~\cite{radford2021learning} & \val{}{0.88}{0.03} & \val{\bf}{0.38}{0.01} & \val{}{1.98}{0.02} & \val{\bf}{1.08}{0.02} & \val{}{1.48}{0.05}\\
 & CLIP (temp. scaling) & \val{}{0.93}{0.03} & \val{\bf}{0.38}{0.01} & \val{}{2.10}{0.02} & \val{}{1.10}{0.02} & \val{}{1.56}{0.05}\\
\rowcolor{scCyan!30}
\cellcolor{white} & BayesVLM & \val{\bf}{0.86}{0.03} & \val{}{0.38}{0.01} & \val{\bf}{1.95}{0.02} & \val{}{1.08}{0.02} & \val{\bf}{1.46}{0.05}\\\hline
\multirow{5}{*}{ECE} & CLIP~\cite{radford2021learning} & $4.31$ & $1.66$ & $15.95$ & $1.97$ & $8.19$\\
 & CLIP (temp. scaling) & $\bf3.96$ & $\bf0.85$ & $20.02$ & $5.37$ & $11.91$\\
\rowcolor{scCyan!30}
\cellcolor{white} & BayesVLM & $4.49$ & $2.65$ & $\bf15.08$ & $\bf1.72$ & $\bf6.61$\\

\bottomrule
\end{tabular}

==> zeroshot_results/zero_shot_clip_base.tex <==

\begin{tabular}{l|l|ccccccc}
\toprule
Metrics & Methods & \sc Flowers-102 & \sc Food-101 & \sc CIFAR-10 & \sc CIFAR-100 & \sc ImageNet-R & \sc UCF101 & \sc SUN397 \\
\hline
    \multirow{4}{*}{ACC $\uparrow$} & CLIP~\citep{radford2021learning} & \val{\bf}{68.99}{0.5899} & \val{}{80.21}{0.2507} & \val{\bf}{93.61}{0.2446} & \val{\bf}{73.76}{0.4399} & \val{}{74.52}{0.5032} & \val{}{59.82}{0.7971} & \val{}{67.18}{0.3333}\\
 & CLIP (temp. scaling) & \val{\bf}{68.99}{0.5899} & \val{}{80.21}{0.2507} & \val{\bf}{93.61}{0.2446} & \val{\bf}{73.76}{0.4399} & \val{}{74.52}{0.5032} & \val{}{59.82}{0.7971} & \val{}{67.18}{0.3333}\\
 & TTA~\citep{farina2024frustratingly} & \val{\bf}{68.87}{0.5905} & \val{\bf}{81.68}{0.2435} & \val{}{88.54}{0.3185} & \val{}{65.64}{0.4749} & \val{\bf}{78.29}{0.4760} & \val{\bf}{63.07}{0.7847} & \val{\bf}{68.58}{0.3295}\\
\rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM  & \val{\bf}{68.87}{0.5905} & \val{}{80.36}{0.2500} & \val{\bf}{93.63}{0.2442} & \val{\bf}{73.65}{0.4405} & \val{}{74.37}{0.5041} & \val{}{61.56}{0.7909} & \val{}{66.92}{0.3339}\\\hline
\cellcolor{white} & BayesVLM
  & \val{\bf}{68.87}{0.4630}   % flowers102
  & \val{}{80.43}{0.3968}      % food101
  & \val{\bf}{93.62}{0.2444}   % cifar10
  & \val{\bf}{73.63}{0.4406}   % cifar100
  & \val{}{74.45}{0.4361}      % imagenet-r
  & \val{}{61.43}{0.4868}      % ucf101
  & \val{}{66.96}{0.4703}      % sun397
\\\hline
    \multirow{4}{*}{NLPD $\downarrow$} & CLIP~\citep{radford2021learning} & \val{}{1.90}{0.0486} & \val{}{0.70}{0.0094} & \val{}{0.21}{0.0079} & \val{}{0.97}{0.0173} & \val{}{1.07}{0.0237} & \val{}{1.59}{0.0366} & \val{}{1.16}{0.0131}\\
 & CLIP (temp. scaling) & \val{\bf}{1.67}{0.0373} & \val{}{0.69}{0.0073} & \val{}{0.21}{0.0061} & \val{\bf}{0.94}{0.0138} & \val{}{1.04}{0.0191} & \val{}{1.46}{0.0282} & \val{\bf}{1.11}{0.0100}\\
 & TTA~\citep{farina2024frustratingly}  & \val{}{1.86}{0.0475} & \val{\bf}{0.67}{0.0094} & \val{}{0.35}{0.0092} & \val{}{1.26}{0.0178} & \val{\bf}{0.90}{0.0210} & \val{}{1.50}{0.0363} & \val{}{1.14}{0.0131}\\
\rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM  & \val{}{1.73}{0.0405} & \val{\bf}{0.68}{0.0079} & \val{\bf}{0.20}{0.0067} & \val{}{0.95}{0.0152} & \val{}{1.03}{0.0203} & \val{\bf}{1.43}{0.0296} & \val{}{1.12}{0.0109}\\\hline
\cellcolor{white} & BayesVLM
  & \val{}{1.73}{0.0320}   % flowers102
  & \val{\bf}{0.68}{0.0126} % food101
  & \val{\bf}{0.20}{0.0067} % cifar10
  & \val{}{0.95}{0.0152}    % cifar100
  & \val{}{1.03}{0.0177}    % imagenet-r
  & \val{\bf}{1.44}{0.0183} % ucf101
  & \val{}{1.12}{0.0155}    % sun397
\\\hline
\multirow{4}{*}{ECE $\downarrow$} & CLIP~\citep{radford2021learning} & $6.59$ & $3.91$ & $1.45$ & $6.31$ & $5.20$ & $11.52$ & $8.71$\\
 & CLIP (temp. scaling) & $5.51$ & $4.74$ & $1.88$ & $3.07$ & $4.80$ & $3.61$ & $2.67$\\
 & TTA~\citep{farina2024frustratingly}  & $9.63$ & $4.18$ & $2.02$ & $5.27$ & $2.88$ & $11.75$ & $9.92$\\
\rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM & $\bf4.32$ & $\bf1.91$ & $\bf0.72$ & $\bf1.77$ & $\bf1.88$ & $\bf3.57$ & $\bf1.77$\\
\cellcolor{white} & BayesVLM
  & $\bf4.22$  % flowers102  (0.04216 ×100)
  & $\bf1.69$  % food101    (0.01687 ×100)
  & $\bf0.72$  % cifar10    (0.00722 ×100)
  & $\bf1.92$  % cifar100   (0.01917 ×100)
  & $\bf1.78$  % imagenet-r (0.01778 ×100)
  & $\bf3.57$  % ucf101    (0.03568 ×100)
  & $\bf2.06$  % sun397    (0.02061 ×100)
\\
\bottomrule
\end{tabular}
    

==> zeroshot_results/zero_shot_clip_large.tex <==

\begin{tabular}{l|l|ccccccc}
\toprule
Metrics & Methods & \sc Flowers-102 & \sc Food-101 & \sc CIFAR-10 & \sc CIFAR-100 & \sc ImageNet-R & \sc UCF101 & \sc SUN397 \\
\hline
    \multirow{4}{*}{ACC $\uparrow$} & CLIP~\citep{radford2021learning} & \val{\bf}{72.04}{0.5723} & \val{}{86.60}{0.2144} & \val{\bf}{95.57}{0.2058} & \val{\bf}{76.74}{0.4225} & \val{}{85.51}{0.4065} & \val{\bf}{69.60}{0.7479} & \val{}{71.48}{0.3205}\\
 & CLIP (temp. scaling) & \val{\bf}{72.04}{0.5723} & \val{}{86.60}{0.2144} & \val{\bf}{95.57}{0.2058} & \val{\bf}{76.74}{0.4225} & \val{}{85.51}{0.4065} & \val{\bf}{69.60}{0.7479} & \val{}{71.48}{0.3205}\\
 & TTA~\citep{farina2024frustratingly}  & \val{}{71.85}{0.5735} & \val{\bf}{87.11}{0.2109} & \val{}{92.83}{0.2580} & \val{}{71.56}{0.4511} & \val{\bf}{87.64}{0.3800} & \val{\bf}{70.10}{0.7443} & \val{\bf}{71.99}{0.3187}\\
 \rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM  & \val{\bf}{72.55}{0.5691} & \val{\bf}{87.18}{0.2104} & \val{\bf}{95.51}{0.2071} & \val{\bf}{76.76}{0.4224} & \val{}{85.65}{0.4048} & \val{\bf}{70.16}{0.7439} & \val{}{71.06}{0.3219}\\\hline
\cellcolor{white} & BayesVLM
  & \val{\bf}{72.42}{0.4469}   % flowers102  (0.72418 ±0.44693)
  & \val{\bf}{87.20}{0.3341}   % food101    (0.87196 ±0.33413)
  & \val{\bf}{95.49}{0.2075}   % cifar10    (0.95490 ±0.20752)
  & \val{\bf}{76.77}{0.4223}   % cifar100   (0.76770 ±0.42230)
  & \val{}{85.63}{0.3508}      % imagenet-r (0.85627 ±0.35082)
  & \val{\bf}{70.26}{0.4571}   % ucf101     (0.70262 ±0.45711)
  & \val{}{71.12}{0.4532}      % sun397     (0.71118 ±0.45321)
\\\hline
\multirow{4}{*}{NLPD $\downarrow$} & CLIP~\citep{radford2021learning} & \val{}{1.75}{0.0479} & \val{}{0.48}{0.0083} & \val{\bf}{0.15}{0.0072} & \val{}{0.90}{0.0178} & \val{}{0.58}{0.0174} & \val{}{1.36}{0.0391} & \val{}{1.02}{0.0128}\\
 & CLIP (temp. scaling) & \val{\bf}{1.51}{0.0378} & \val{}{0.47}{0.0065} & \val{\bf}{0.15}{0.0056} & \val{\bf}{0.87}{0.0143} & \val{}{0.59}{0.0144} & \val{\bf}{1.20}{0.0298} & \val{\bf}{0.96}{0.0098}\\
 & TTA~\citep{farina2024frustratingly}  & \val{}{1.74}{0.0472} & \val{}{0.49}{0.0086} & \val{}{0.24}{0.0080} & \val{}{1.15}{0.0188} & \val{\bf}{0.49}{0.0160} & \val{}{1.34}{0.0390} & \val{}{1.06}{0.0133}\\
 \rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM & \val{}{1.62}{0.0424} & \val{\bf}{0.45}{0.0068} & \val{\bf}{0.15}{0.0060} & \val{\bf}{0.87}{0.0155} & \val{}{0.57}{0.0152} & \val{}{1.22}{0.0329} & \val{}{0.98}{0.0109}\\\hline
\cellcolor{white} & BayesVLM
  & \val{}{1.62}{0.0335}   % flowers102  (3.3481 → 0.0335)
  & \val{\bf}{0.45}{0.0110} % food101     (1.0951 → 0.0110)
  & \val{\bf}{0.15}{0.0061} % cifar10     (0.6074 → 0.0061)
  & \val{\bf}{0.87}{0.0155} % cifar100    (1.5507 → 0.0155)
  & \val{}{0.57}{0.0132}    % imagenet-r  (1.3214 → 0.0132)
  & \val{}{1.22}{0.0204}    % ucf101      (2.0357 → 0.0204)
  & \val{}{0.98}{0.0154}    % sun397      (1.5395 → 0.0154)
\\\hline
\multirow{4}{*}{ECE $\downarrow$} & CLIP~\citep{radford2021learning} & $9.47$ & $3.07$ & $0.97$ & $5.73$ & $2.13$ & $10.72$ & $8.60$\\ 
 & CLIP (temp. scaling) & $4.90$ & $3.00$ & $1.35$ & $2.55$ & $5.21$ & $\bf3.40$ & $\bf1.48$\\
 & TTA~\citep{farina2024frustratingly}  & $11.96$ & $3.77$ & $1.21$ & $3.92$ & $\bf1.92$ & $11.87$ & $10.53$\\  \rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM & $\bf4.17$ & $\bf1.20$ & $\bf0.63$ & $\bf1.89$ & $2.48$ & $5.23$ & $3.61$\\
\cellcolor{white} & BayesVLM
  & $\bf4.66$  % flowers102  (0.04664 ×100)
  & $\bf1.00$  % food101    (0.00999 ×100)
  & $\bf0.62$  % cifar10    (0.00618 ×100)
  & $\bf1.91$  % cifar100   (0.01911 ×100)
  & $2.15$     % imagenet-r (0.02150 ×100)
  & $5.37$     % ucf101    (0.05369 ×100)
  & $3.89$     % sun397    (0.03890 ×100)
\\
\bottomrule
\end{tabular}
    

==> zeroshot_results/zero_shot_laion_vs_cc12m.tex <==
\begin{tabular}{l|l|ccccccc}
\toprule
Metrics & Dataset & \sc Flowers-102 & \sc Food-101 & \sc CIFAR-10 & \sc CIFAR-100 & \sc ImageNet-R & \sc UCF101 & \sc SUN397 \\
\hline
\multirow{2}{*}{ACC $\uparrow$}
  & LAION-400M
    & \val{\bf}{68.87}{0.4630} & \val{}{80.43}{0.3968} & \val{}{93.62}{0.2444} & \val{}{73.63}{0.4406} & \val{}{74.45}{0.4361} & \val{}{61.43}{0.4868} & \val{}{66.96}{0.4703} \\
  & CC12M
    & \val{}{68.12}{0.4660} & \val{}{80.35}{0.3974} & \val{}{93.57}{0.2453} & \val{}{73.78}{0.4398} & \val{}{74.32}{0.4369} & \val{}{61.46}{0.4867} & \val{}{66.81}{0.4709} \\
\hline
\multirow{2}{*}{NLPD $\downarrow$}
  & LAION-400M
    & \val{\bf}{1.73}{0.0320} & \val{}{0.68}{0.0126} & \val{}{0.20}{0.0067} & \val{}{0.95}{0.0152} & \val{\bf}{1.03}{0.0177} & \val{}{1.44}{0.0183} & \val{\bf}{1.12}{0.0155} \\
  & CC12M
    & \val{}{1.77}{0.0330} & \val{}{0.68}{0.0129} & \val{}{0.20}{0.0067} & \val{}{0.95}{0.0152} & \val{}{1.03}{0.0180} & \val{}{1.44}{0.0185} & \val{}{1.13}{0.0162} \\
\hline
\multirow{2}{*}{ECE $\downarrow$}
  & LAION-400M
    & $4.22$ & $1.69$ & $0.72$ & $1.92$ & $1.78$ & $\bf3.77$ & $\bf2.06$ \\
  & CC12M
    & $\bf3.84$ & $\bf0.99$ & $\bf0.70$ & $\bf1.43$ & $\bf1.39$ & $3.83$ & $3.89$\\
\bottomrule
\end{tabular}

==> zeroshot_results/zero_shot_siglip_base.tex <==

\begin{tabular}{l|l|ccccccc}
\toprule
Metrics & Methods & \sc Flowers-102 & \sc Food-101 & \sc CIFAR-10 & \sc CIFAR-100 & \sc ImageNet-R & \sc UCF101 & \sc SUN397 \\
\hline
    \multirow{4}{*}{ACC $\uparrow$} & SigLIP~\citep{zhai2023sigmoid} & \val{\bf}{82.31}{0.4867} & \val{}{88.81}{0.1984} & \val{\bf}{93.20}{0.2517} & \val{\bf}{71.27}{0.4525} & \val{}{89.71}{0.3509} & \val{\bf}{59.61}{0.7978} & \val{\bf}{67.55}{0.3323}\\
 & SigLIP (temp. scaling) & \val{\bf}{82.31}{0.4867} & \val{}{88.81}{0.1984} & \val{\bf}{93.20}{0.2517} & \val{\bf}{71.27}{0.4525} & \val{}{89.71}{0.3509} & \val{\bf}{59.61}{0.7978} & \val{\bf}{67.55}{0.3323}\\
 & TTA~\citep{farina2024frustratingly}  & \val{\bf}{82.66}{0.4828} & \val{\bf}{89.24}{0.1950} & \val{}{87.96}{0.3254} & \val{}{60.95}{0.4879} & \val{\bf}{90.91}{0.3320} & \val{\bf}{60.14}{0.7960} & \val{}{66.82}{0.3342}\\
% \rowcolor{scCyan!30} \cellcolor{white} & BayesVLM & \val{\bf}{82.21}{0.4877} & \val{}{88.75}{0.1988} & \val{\bf}{93.20}{0.2517} & \val{\bf}{71.28}{0.4525} & \val{}{89.73}{0.3505} & \val{\bf}{59.48}{0.7982} & \val{\bf}{67.59}{0.3322}\\\hline
\rowcolor{scCyan!30} \cellcolor{white} & BayesVLM
  & \val{\bf}{82.44}{0.3805}   % flowers102  (0.82436 ±0.38051)
  & \val{}{88.84}{0.3148}      % food101    (0.88844 ±0.31483)
  & \val{\bf}{93.16}{0.2524}   % cifar10    (0.93160 ±0.25243)
  & \val{\bf}{71.22}{0.4527}   % cifar100   (0.71220 ±0.45274)
  & \val{}{89.72}{0.3037}      % imagenet-r (0.89720 ±0.30370)
  & \val{\bf}{59.69}{0.4905}   % ucf101     (0.59688 ±0.49052)
  & \val{\bf}{67.44}{0.4686}   % sun397     (0.67441 ±0.46860)
\\\hline
\multirow{4}{*}{NLPD $\downarrow$} & SigLIP~\citep{zhai2023sigmoid} & \val{}{0.88}{0.0285} & \val{}{0.38}{0.0061} & \val{\bf}{0.21}{0.0063} & \val{\bf}{1.08}{0.0168} & \val{}{0.41}{0.0139} & \val{}{1.90}{0.0438} & \val{}{1.12}{0.0117}\\
 & SigLIP (temp. scaling) & \val{\bf}{0.84}{0.0246} & \val{}{0.40}{0.0054} & \val{}{0.22}{0.0057} & \val{}{1.09}{0.0152} & \val{}{0.43}{0.0125} & \val{\bf}{1.77}{0.0376} & \val{}{1.12}{0.0102}\\
 & TTA~\citep{farina2024frustratingly}  & \val{\bf}{0.85}{0.0276} & \val{\bf}{0.37}{0.0064} & \val{}{0.36}{0.0073} & \val{}{1.62}{0.0209} & \val{\bf}{0.37}{0.0134} & \val{}{1.88}{0.0430} & \val{}{1.18}{0.0124}\\
\rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM & \val{}{0.85}{0.0263} & \val{}{0.40}{0.0055} & \val{}{0.21}{0.0060} & \val{\bf}{1.08}{0.0159} & \val{}{0.42}{0.0128} & \val{}{1.79}{0.0387} & \val{\bf}{1.11}{0.0105}\\\hline
\cellcolor{white} & BayesVLM
  & \val{}{0.86}{0.0210}   % flowers102  (2.1028 → 0.0210)
  & \val{}{0.39}{0.0091}   % food101    (0.9055 → 0.0091)
  & \val{\bf}{0.21}{0.0061}   % cifar10    (0.6077 → 0.0061)
  & \val{\bf}{1.08}{0.0163} % cifar100   (1.6251 → 0.0163)
  & \val{}{0.41}{0.0114}   % imagenet-r (1.1406 → 0.0114)
  & \val{}{1.82}{0.0248}   % ucf101     (2.4762 → 0.0248)
  & \val{\bf}{1.12}{0.0154} % sun397    (1.5352 → 0.0154)
\\\hline
\multirow{4}{*}{ECE $\downarrow$} & SigLIP~\citep{zhai2023sigmoid} & $\bf4.31$ & $1.66$ & $\bf0.92$ & $1.97$ & $\bf1.36$ & $12.72$ & $3.82$\\
 & SigLIP (temp. scaling) & $6.28$ & $5.54$ & $2.94$ & $4.47$ & $4.85$ & $\bf6.69$ & $2.83$\\
 & TTA~\citep{farina2024frustratingly}  & $4.56$ & $\bf0.72$ & $3.14$ & $2.09$ & $1.59$ & $13.47$ & $6.81$\\
\rowcolor{scCyan!30}
% \cellcolor{white} & BayesVLM  & $5.10$ & $4.87$ & $1.82$ & $\bf1.79$ & $3.96$ & $7.87$ & $\bf1.09$\\
\cellcolor{white} & BayesVLM
  & $4.87$  % flowers102  (0.04867 ×100)
  & $3.49$  % food101    (0.03492 ×100)
  & $1.38$  % cifar10    (0.01380 ×100)
  & $\bf1.52$  % cifar100   (0.01516 ×100)
  & $2.79$  % imagenet-r (0.02790 ×100)
  & $9.60$  % ucf101    (0.09605 ×100)
  & $\bf1.14$  % sun397    (0.01142 ×100)
\\

\bottomrule
\end{tabular}
    
